Ad Astra White Paper: A Pitch for the Next 25 Years of NASA's Physics of the Cosmos Program

Astrophysical observations of our universe have been key to our understanding of how the universe works. Shortly after the turn of the millennium, the National Research Council delivered \textit{Connecting Quarks with the Cosmos: Eleven Science Questions for the New Century}. In the subsequent quarter-century, we have made substantial progress in answering each question. These advancements have, in part, arisen because of the success of major US facilities across several domains of physics, guided by long-term planning documents which still largely focus on these questions. This report seeks to provide a status update on each question, and to outline what space-based facilities are crucial for future progress, intended to guide NASA's preparatory work for the Astro2030 Decadal.

==> authors.tex <==
\author[0000-0002-2942-3379]{Eric Burns}
\affiliation{Department of Physics \& Astronomy, Louisiana State
University, Baton Rouge, LA 70803, USA}
\email{ericburns@lsu.edu}




